RedKnot: Efficient Long-Context LLM Serving with Head-Aware KV Reuse and SegPagedAttention

As the input length of large language model (LLM) serving continues to grow, the KV cache has become a dominant bottleneck in AI infrastructure. It limits GPU memory capacity, serving concurrency, cache reuse, and distributed scalability. Multiple important problems, including position-independent KV cache, prefix KV cache compression, hot/cold KV cache separation, and distributed KV cache management, all depend on how the KV cache is represented and managed. However, existing serving systems largely rely on a monolithic KV cache abstraction, where the KV cache is treated as a homogeneous sequence of token-level memory blocks and managed with similar policies across attention heads and serving scenarios. We observe that KV cache utility is highly structured across KV heads: different heads exhibit different functional roles, attention distances, and runtime importance. Therefore, a full KV cache is not always necessary for every head, token range, or serving scenario. We present RedKnot, a head-aware KV cache management system for LLM serving. RedKnot breaks the conventional monolithic KV cache abstraction by decomposing the KV cache along KV heads, whose importance and effective attention ranges vary significantly across serving scenarios. This head-level decomposition turns the KV cache from a monolithic tensor abstraction into a structured memory object, enabling RedKnot to uniformly support position-independent KV reuse, prefix KV compression, hot/cold KV separation, and distributed KV placement while preserving output fidelity and improving resource efficiency, without requiring model retraining or fine-tuning. RedKnot establishes a new foundation for AI infrastructure by transforming the KV cache from a monolithic, passive runtime artifact into a dynamic, model-aware runtime substrate for scalable LLM serving.

==> sections/Motiv_V2.tex <==
\section{Limitation and Motivation}\label{sec3.1}
%
Building on the previous section, we further analyze the limitations of PDC and PIC in agentic settings (\S3.1). We then diagnose their root causes and report preliminary mitigation experiments (\S3.2); guided by these results, we introduce a new caching paradigm (\S3.3).
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Limitations of PDC and PIC In Agentic Prompts}\label{LimitofPIC&PDC}
%
\noindent Under the agentic prompt setting in section~\ref{back_2}, mainstream \textbf{PDC} methods  assume fixed absolute positions for reusable segments.~This implies that, as update segments vary in length, ContextCache can only reuse identical prompt prefixes and even if one swaps the order of updated segments and fixed segments,as shown in Figure~\ref{fig:back_2}~\ding{172}, we cannot simply swap the fixed and updated segments and reuse the KVCache via prefix caching, Since the prompt head generally attracts more attention~\cite{attention_head,attention_head_1}, representative designs (e.g., MemGPT) position recent memories(Working Window) close to the head instead of FIFO historical content to maintain inference quality.~Similarly, in SWE-agent a widely used code-debugging agent with multiple updated slots~\ding{173} the updated slots cannot be swapped with immutable segments~\ding{174}, as such reordering changes program semantics and breaks data dependencies  (e.g., if Updated Slot 1 produces a run-time parameter later consumed by Immutable 1, moving the slot to the suffix prevents Immutable 1 from receiving it).  Turning to PromptCache, it must precompute and store per-segment KVCaches in isolation (capturing only intra-segment attention) and, upon reuse, does not restore cross-attention either among reused segments or between reused and updated segments, thereby proliferating KVCache versions and incurring substantial storage overhead.~In short,Strict absolute-position constraints render PDC of limited utility in agent scenarios.\\
\indent By contrast, mainstream \textbf{PIC} methods abandon absolute coordinates and reset reused segments' starting indices to zero, thereby inducing positional/attention misalignment between the cached KVs and those recomputed from scratch at their intended positions in the input.~To partially recover accuracy, these methods \emph{preselect a subset of tokens} from the KVcache for recomputing.~However, in multi-head attention of transformer, different heads attend to different tokens, and the model’s output is fusing  the per-head results~\cite{mutil-head_2,mutil-head}.
% ~During decoding, the set of heads that contribute most to the output varies with the context at each step~\cite{mutil-head_3,mutil-head_4}.
~Since which tokens most affect the output becomes clear only at the decoding stage, prefill-phase token-subset preselection cannot ensure stable accuracy.\\
\textbf{From a systems standpoint}, ~the implementation of PIC entails loading the KVCache and writing the recomputed KVs for the selected tokens on a layer-wise basis. ~However,~mainstream LLM inference frameworks(eg. vLLM~\cite{vLLM},SGLang~\cite{sglang}, TensorRT-LLM~\cite{TensorRTLLM}) serialize KVCache loads and writes at each layer. ~This leads to a \emph{load-before-write lock} within the layer, eliminating intra-layer overlap and yielding I/O-bound stalls on the prefill critical path. ~When capacity pressure forces KVCache pages to spill to SSDss, current mainstream systems (e.g.,  vLLM,SGLang, TensorRT-LLM,LMDeploy~\cite{lmdeploy_github}) treat pages  typically evict KV blocks via LRU rather than dirty-aware scheme; consequently, partially updated pages incur random writes and higher write amplification (WAF) on eviction. Lacking dirty-aware eviction or write coalescing, these I/O costs propagate to the prefill path, worsening I/O-bound stalls and tail latency. ~Though PIC offers positional flexibility, it comes at the high cost of attention misalignment and non-trivial system overhead.\\
\indent Taken together, both the accuracy degradation and the system inefficiencies of PDC/PIC stem from the same root cause: \emph{positional misalignment}. In particular, when reusable segments shift in absolute position, their cached KVs no longer match the recomputed ones, leading to attention misalignment. We denote this divergence as \textbf{Positionally Misaligned KV Drift (PMKD)}.
% 
\begin{figure}[t]
\includegraphics[width=0.98\linewidth]{sections/figures/section 3/PMKD&Padding.pdf}
  \caption{(a) shows that as the positional shift increases (0–1000 tokens), CKSim with RoPE drops by $>90\%$, whereas CKSim with CoPE decreases by only 28\%. (b) shows that applying window padding(1K/2K/3K) yields $>78.1\%$ lower F1 score relative to baseline inference at the same reasoning rounds.}
   \vspace{-2ex}
  \label{fig:expofCKsim}
\end{figure}
%
\subsection{Quantifying PMKD and Window Padding}\label{sec:PMKD_and window_padded}
%
Building on above, we now quantify PMKD by measuring the effect of controlled positional shifts on KVs obtained by recomputation and by reuse, using two widely used positional encodings: RoPE (high positional sensitivity) and CoPE (low positional sensitivity) as discussed in Section~\ref{back_2}. This contrast isolates the role of positional encoding in PMKD and shows how sensitivity governs KV drift under absolute shifts.~We adopt CKSim~\cite{CKV_1,CKV_2}, the standard cosine-similarity metric for measuring the similarity between two KVs, the expression is as follows:
\[
\mathrm{CKSim}(reuse,recompute)=\frac{1}{H}\sum_{i=1}^{H}\frac{K_i^{(\mathrm{recompute})}\cdot K_i^{(\mathrm{reuse})}}{\lVert K_i^{(\mathrm{recompute})}\rVert\lVert K_i^{(\mathrm{reuse})}\rVert}
\]
\noindent In the above definition, $K_{i}^{(\mathrm{recompute})}$ denotes the key matrix for head $i$ obtained by recomputing and $K_{i}^{(\mathrm{reuse})}$ denotes the key matrix for head $i$ obtained by reusing. Each key matrix $K$ encodes positional information through the model’s positional encoding. The symbol $H$ denotes the number of attention heads. We use $\mathrm{CKSim}$ to quantify the similarity between two segments’ $K$ matrices; the corresponding similarity computed on the $V$ matrices closely tracks that of $K$ matrix.\\
\indent We evaluate CKSim by MemGPT~\cite{MemGPT} on ShareGPT~\cite{ShareGPT} dataset by constructing, for a each user, a static historic memory(MemHistory). ~We proceed as follows:
\begin{enumerate}
  \item Using RoPE, encode MemHistory and obtain the baseline KVCache as \emph{KVCache 0}.
  \item For prefix window(i.e., the length of the context preceding MemHistory) sizes \(i \in \{100,200,300,\ldots\}\) (step size: 100 tokens),  prepend a prefix of length \(i\) to MemHistory and run a partial prefill(Only the positional information of MemHistory is prefilling; attention on the prefix is not computed) to obtain \emph{KVCache i}.
  \item Compute \(\mathrm{CKSim}\) between  \emph{KVCache i} and \emph{KVCache 0}.
  \item Replace RoPE with CoPE and repeat steps~(1)--(3).
\end{enumerate}
%
\begin{figure}[t]
  \includegraphics[width=0.98\linewidth]{sections/figures/section 3/PMKD.pdf}
  \caption{Compared with RoPE, CoPE achieves better alignment between cached and real positions during KVCache reuse, yielding a shallower mapping slope and thereby substantially reducing the positional discrepancy  ($\Delta \mathrm{pos}$ ).}
   \vspace{-3ex}
  \label{fig:PMKD_and_padding}
\end{figure}
%
\indent As shown in Figure~\ref{fig:expofCKsim}~(a), we observe that RoPE exhibits a more pronounced decline in CKSim, whereas CoPE maintains comparatively stable CKSim. ~We define \textbf{Positionally Misaligned KV Drift(PMKD)} as the discrepancy in KVCache similarity  for the same text that is attributable to differences in positional encodings.~As shown in Figure~\ref{fig:PMKD_and_padding}~\ding{172},when the length of the update segment changes, the real positional indices of the fixed segment can diverge substantially from those stored in the KVCache, because RoPE assigns a position index to every token(For example, after the update, the true starting positions in the KVCache are 251 and 451, whereas the cached positions remain at 101 and 401). ~Under the same update length, CoPE markedly reduces the positional offset of the fixed segment. For example, in Figure~\ref{fig:PMKD_and_padding}~\ding{173}, the offset $\Delta\mathrm{pos}$ decreases, with the fixed segment’s starting positions shifting from (10, 21) to (9, 20). ~At a deeper reason, as shown in Figure ~\ref{fig:PMKD_and_padding}~\ding{174}, when the starting positions of one context shift, RoPE exhibits a steeper change in positional indices because it maps each token to a unique position, whereas CoPE varies more smoothly since multiple tokens can share a single position.~Since attention is jointly determined by positional information and content, if the cached tokens of a fixed segment attend either to tokens within the same segment or to tokens in other fixed segments, then maintaining a high CKSim  affords a key opportunity: near-lossless reuse of both intra-segment attention within fixed segments and cross-segment attention among fixed segments.~Therefore, reducing PMKD and maintaining KV consistency are crucial to achieving high-quality cache reuse.~A commonly used and straightforward mitigation strategy is window padding.\\
\noindent \textbf{Window Padding:}~That minimizing absolute positional changes is crucial for KVCache reuse, a natural approach is to bound the variation in the length of each dynamic update segment, thereby constraining the positional drift of fixed segments at the source.~So we can bound positional drift by fixing the update-span length via a \emph{window padding} policy.~So we enforce a fixed-size update window for the updated segments (capping its max token count),~so that the positions of the fixed segments  remain invariant, as shown in Figure~\ref{fig:PMKD_and_padding}~\ding{172} window padding. ~Using popular agent MemGPT, we fix the  working window to 1K,2K and 3K tokens, after multiple reasoning rounds (as shown in Figure~\ref{fig:expofCKsim}~(b)), window-padded inference attains markedly lower accuracy than the baseline inference(not set window-padded), indicating that enforcing a fixed-length update segment can cause the loss of critical information across inferences(working window=1K) or larger window(working window=3K) padding increases the PMKD of the fixed segment’s KVCache.~In window-padded experiments, in real-world agentic scenarios, it is hard to find a suitable window size.~Since the token counts of the updated segments in multi-agent inputs show large and unpredictable fluctuations~\cite{length_fluctuations,length_fluctuations_1,length_fluctuations_2}.\\
\textbf{Summary.}The smaller the positional misalignment between cached and recomputed KVs, the higher their similarity—enabling \emph{near-lossless} reuse of both intra-segment attention within fixed segments and cross-segment attention involving fixed segments. ~However,  window padding alone rarely achieves this objective in practice.%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Relative-Position-Dependent Caching}\label{PRDC}
% Building on above, keeping the positional discrepancy between cached and recomputed KVs small enables near-lossless reuse of fixed segments preserving both intra-segment and cross-segment attention,~so that only the cross-attention between fixed and updated segments must be recovered. Evidently, this requires recomputing a subset of tokens from the fixed segments, which inherits the same system-level limitations as PIC methods.~We introduce a new KVCache reuse paradigm, \emph{Relative-Position-Dependent Caching (RPDC)}, which is fundamentally distinct from PDC and PIC(\S 2.3).~In the next section, we present CacheSlide, a system that implements RPDC.%
%
\begin{figure*}[t] % 星号(*)表示跨双栏
  \centering
  \includegraphics[width=0.95\textwidth]{sections/figures/section 4/OverView.pdf} % 调整width比例适应页面
  \caption{Block diagram of proposed CacheSlide system workflow} % 标题描述
  \label{fig:system_overview} % 引用标签
\end{figure*}
%
Motivated by the above, we introduce Relative-Position-Dependent Caching (RPDC), a new KVCache reuse paradigm fundamentally distinct from PDC and PIC (\S 2.3). RPDC preserves the relative ordering of reusable segments so that the positional discrepancy between cached and from-scratch KVs remains small. As a result, intra-segment and cross-fixed-segment attention can be reused near-losslessly; only the cross-attention between fixed and updated segments needs to be recovered by recomputing a subset of tokens in the fixed segments, but this inherits PIC-like system limitations(\S 3.1). In the next section, we present CacheSlide, a system that implements RPDC efficiently.
%


==> sections/ack.tex <==
% \section*{Acknowledgments}
% %
% We would like to thank the anonymous reviewers and our shepherd Petros Maniatis
% for their valuable feedback.
% %
% This work was supported in part by a research grant from Samsung Advanced
% Institute of Technology (SAIT) and by the artificial intelligence semiconductor
% support program to nurture the best talents (No. RS-2023-00256081) supervised
% by Institute for Information \& Communications Technology Planning \&
% Evaluation (IITP).
% %
% The Institute of Engineering Research at Seoul National University provided
% research facilities for this work.
% %
% Jaewoong Sim is the corresponding author.


==> sections/discussion.tex <==
\putsec{discussion}{Analysis and Discussion}
\putssec{sensitivity}{Sensitivity Study}
%
We use the OPT-6.7B model with 1920 input tokens, 128 output tokens, and a
batch size of 8. The accuracy is evaluated with the WinoGrande task in
lm-evaluation-harness.

\begin{figure}[t]
  \includegraphics[width=\linewidth]{figures/alpha_sweep.pdf}
  \caption{
    Accuracy and inference latency across (a) alpha values and (b) partial
    weight ratios.
  }
  \vspace{-0.15in}
  \label{fig:alpha_sweep}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\myparagraph{Threshold and Alpha.}
%
As discussed in~\ssecref{prefetching}, we load the KV cache of the tokens with
a speculated attention score greater than the threshold (i.e., the maximum
attention score minus alpha). Increasing alpha results in fetching more KV
entries to the GPU, thus increasing inference latency but also improving
accuracy.
%
\figref{alpha_sweep}(a) shows such trade-offs between accuracy and inference
latency for nine different alpha values with a partial weight ratio of 0.3. 
%
The results show that more KV entries are fetched and involved in attention
computation as alpha increases, thereby leading to better accuracy.
%
For the alpha values beyond 4, however, since most important tokens are already
included, the accuracy does not further increase, while the cost for KV
transfers and attention computation keeps increasing. This trend is similarly
observed in other models, and we thus opt for an alpha value of 4 or 5 to
strike a balance between inference latency and accuracy.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\myparagraph{Partial Weight Ratio.}
%
\figref{alpha_sweep}(b) shows the accuracy and inference latency across
different partial weight ratios with an alpha value of 4. 
%
As shown in the figure, the amount of partial weights has a negligible impact
on inference latency because the cost for computing the speculated attention
score is relatively small. Note that the amount of KV cache to transfer is
\emph{not} related to the partial weight ratio.
%
However, increasing the partial weight ratio results in higher memory
consumption for partial weights and key cache (e.g., doubling the ratio doubles
the memory consumption overhead).
%
The accuracy also does not noticeably differ beyond a ratio of 0.3. In our
work, we opt for a partial weight ratio of 0.3 to achieve better accuracy while
considering memory consumption overhead.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\putssec{}{Overhead}

\begin{figure}[t]
  \includegraphics[clip=True, trim=0in 0.1in 0in 0in, width=\linewidth]{figures/block_latency_breakdown.pdf}
  \caption{
    Latency breakdown of a Transformer block for OPT-13B with a sequence length
    of 2048 and a batch size of 8.
  }
  \vspace{-0.15in}
  \label{fig:block_latency_breakdown}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent\textbf{Prefetching Overhead.}
%
\figref{block_latency_breakdown} shows the latency breakdown of executing a
single Transformer block for the OPT-13B model; FFN is not shown in the figure
for schemes other than Ideal because it is fully overlapped with data transfer
time. Ideal is a scenario where all the computations (i.e., attention and FFN)
are performed on the GPU without any data transfer between the CPU and GPU.
%
As shown in the results, the key performance bottleneck of FlexGen and \ho{} is
the data transfer overhead, which occupies 96.9\% and 91.8\% of the execution
time, respectively.
%
For INT4, due to the quantization and dequantization overhead, attention
computation also occupies a large portion of the execution time in addition to
the data transfer.
%
\name{}, on the other hand, considerably improves the inference speed over
FlexGen by reducing the amount of data transfer with our dynamic KV cache
prefetching. Furthermore, \name{} is only 1.52$\times$ slower than Ideal, while
others show 3.90$\times$-18.55$\times$ slowdowns.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\myparagraph{Memory Consumption.}
%
\name{} uses the partial query weight and key cache for speculation.
% 
For a ratio of 0.3, the sizes of the partial query weight and key cache are
only 2.5\% and 15\% of the total model parameters and total KV cache,
respectively. 
%
While we simply store them in the GPU during our experiments, we can manage the
storage overhead in various optimized ways if needed. For example, we can store
only the column indices of the partial query weight and retrieve the column
vectors from the full query weight matrix (which already resides in the GPU) as
needed for partial query projection. Additionally, we can place the partial key
cache in the CPU and perform speculation on the CPU after fetching the partial
query from the GPU.
%
Even a na\"ive method of lowering the partial ratio would likely still provide
better accuracy compared to other methods while reducing storage overhead.
%
In summary, by minimally sacrificing inference performance, we can greatly
reduce the storage overhead on the GPU if necessary.

\begin{figure}[t]
  \includegraphics[width=\linewidth]{figures/32k_scalability.pdf}
  \caption{
    Perplexity of Llama-2-7B-32K across (a) relative KV cache sizes with a
    sequence length of 32768 and (b) sequence lengths while retaining 64
    tokens.  Lower is better.  Llama-2-7B-32K is a fine-tuned version capable
    of processing up to 32K tokens using position
    interpolation~\cite{che:won23}.  Quantization is omitted in (b) since the
    KV cache cannot be compressed below 6.25\% (i.e., 1 bit).
  }
  \vspace{-0.15in}
  \label{fig:scalability}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\putssec{}{Long Context Window}
%
\figref{scalability} shows the perplexity of the Llama-2-7B-32K model, which
can process up to 32K tokens, across the relative cache sizes and sequence
lengths.
%
We use the WikiText-2 dataset for the experiment.
%
As the context window size increases for future LLMs, the relative portion of
the KV cache that the GPU can retain would decrease due to the limited capacity
of GPU memory.

\figref{scalability}(a) shows that \name{} maintains perplexity levels close to
the full-cache baseline even as the relative KV cache size decreases, without
leading to a noticeable increase in perplexity even with much smaller cache
sizes.
%
In contrast, other methods increase perplexity compared to the full-cache
baseline and significantly diverge at certain sizes due to insufficient bit
widths for preserving adequate information on all keys and values
(Quantization) or the permanent removal of KV cache entries (\ho{}).
%
As shown in~\figref{scalability}(b), the perplexity gap between \name{} and
\ho{} widens for longer sequence lengths, which is likely to increase further
for sequence lengths beyond 32K. This implies that \name{} can scale to longer
sequences and better preserve model accuracy compared to others.

\begin{figure}[t]
  \includegraphics[width=\linewidth]{figures/1m_scalability.pdf}
  \caption{
    Analysis of 1 million tokens using Llama-3-8B-1048K. (a) Percentage of
    query tokens that attend to less than 1\% of the key tokens across the
    sequence lengths. (b) Attention weight of sampled key tokens from different
    layers and heads across the last 16K iterations out of 1 million tokens.
  }
  \vspace{-0.15in}
  \label{fig:1m}
\end{figure}

We further speculate on how \name{} would benefit in an era of million-token
context windows by analyzing a model capable of handling 1 million tokens. 
%
\figref{1m}(a) shows that the percentage of query tokens that attend to less
than 1\% of key tokens increases as the sequence length becomes longer. 
%
\name{} can adapt to this changing trend by dynamically adjusting the amount of
the KV cache to load, whereas prior fixed-budget/pruning approaches would not
easily adjust the effective KV cache size.
%
\figref{1m}(b) further shows that the attention weights of key tokens can
change across iterations; the sampled key tokens show sudden \emph{spikes}
after thousands of iterations with significantly low attention weights (e.g.,
the 7425{$^\textrm{th}$} iteration out of the last 16K iterations in Layer 18,
Head 30).
%
We observe that the prior approaches that permanently eliminate tokens while
they are unimportant could lose the critical contexts if they become important
again at later iterations. 
%
In contrast, \name{} can preserve model performance by keeping the temporarily
unimportant KV entries for potential future use.


==> sections/disign.tex <==
\section{CacheSlide Design}\label{sec4}
% ---------------------------  TABLE  ---------------------------------
% \begin{table}[t]
%   \caption{Explanation of Key Terminology}
%   \label{tab:attn_explain}
%   \centering
%   \begin{tabularx}{\textwidth}{@{\extracolsep{\fill}}lX}
%     \toprule
%     \textbf{Attention Mechanism} & \textbf{Principle and Characteristics} \\ \midrule
%     Local Attention &
%     Attention weights are computed only within a sliding window (or predefined block) of length $k$, leading to computational and memory complexity of $\mathcal{O}(nk)$.  
%     This design substantially reduces latency and memory footprint for long sequences and excels at capturing short-range dependencies;  
%     however, information outside the window must propagate through subsequent layers, which lowers the efficiency of modeling long-range dependencies. \\

%     Full Attention  &
%     Each query attends to every key, producing an $n{\times}n$ attention matrix with computational and memory complexity of $\mathcal{O}(n^{2})$.  
%     The resulting dense global connectivity enables a single layer to model long-range dependencies and typically yields stronger performance,  
%     yet the quadratic cost causes prohibitive resource consumption and inference latency on very long sequences. \\ \bottomrule
%   \end{tabularx}
% \end{table}
% % ---------------------------------------------------------------------

In this section, we introduce CacheSlide, a system that addresses the challenges identified in Section~\ref{ChallengesofPRDC}. CacheSlide assigns identical positional encodings to reuse contexts across different LLM inputs, precomputes cross-attention among reuse contexts, and implements relocation and overwriting mechanisms in PagedAttention. Through these innovations, we reduce TTFT, improve storage efficiency, and achieve high effective throughput.
% 
\begin{figure*}[htbp] % 星号(*)表示跨双栏
  \centering
  \includegraphics[width=0.9\textwidth,height=5cm]{sections/figures/section 4/Overview.pdf} % 调整width比例适应页面
  \caption{Block diagram of proposed CacheSlide system workflow} % 标题描述
  \label{fig:system_overview} % 引用标签
\end{figure*}
%
\subsection{Workflow of CacheSlide}
%
We begin by outlining the CacheSlide workflow.~As shown in Figure~\ref{fig:system_overview}~CacheSlide first encodes user inputs with CCPE and applies preprocessing, after which the KV caches of reusable contexts are loaded into the model. Inference accuracy is restored through a Weighted Correction Attention mechanism, and the CacheSlide-optimized PagedAttention subsequently accelerates the workflow.The proposed system integrates task dispatching controller,
cache engine, Weighted Correction Attention and PagedAttention optimization module.
task dispatching controller: The Task Dispatching Controller receives a user prompt, it divides the prompt into chunks based on CCPE. ~As shown in Figure~\ref{fig:system_overview} ~\ding{172} the controller then send reuse chunks to the Cache Management Component and sends the recompute chunks to LLMs as shown in  Figure~\ref{fig:system_overview}~\ding{175}. ~After the LLM completes the current inference, it sends appending KV to KV Cache Store module as shown in Figure~\ref{fig:system_overview}~\ding{176} and  ~\ding{172}. cache engine: 
~The cache engine is a retrieving  KV cache from DRAM and SSD and manage them by computing prompt hash to ensure consistent identification and reuse of the same prompt context.  These retrieved KV are subsequently transmitted to the LLMs for context initialization during the prefill phase as Figure~\ref{fig:system_overview}~\ding{172}, ~\ding{173} and ~\ding{174}. Conversely, when processing an append KV request, the system stores the KV by hash key. The process is schematically illustrated as Figure~\ref{fig:system_overview}~\ding{177}, ~\ding{172} and ~\ding{173}.~Next, we describe the implementation of CacheSlide in detail.
%
\subsection{Chunked Contextual Position Encoding (CCPE)}
To address the positional encoding alignment challenge, we propose Chunked Contextual Position Encoding (CCPE). This technique is inspired by recent works such as CoPE~\cite{Cope}, which maps multiple tokens(e.g. paragraphs or sentences) to a single position rather than one-token-to-one-position like Rope~\cite{Rope}, ABiLi~\cite{alibi} and absolute PE~\cite{ab_PE}. It partitions LLM input into multiple chunks according to reuse-and-recompute criteria and assigns each chunk a fixed positional-encoding range. 


\indent  We explore whether the distinctive properties can be harnessed so that non-reusable contexts exert negligible influence on the positional encodings of reusable contexts.~we use CVsim(section ~\ref{PIKVD})~as a metric to measures how similar a token’s KV remain after its positional encoding is shifted by a specified offset, relative to the token’s original KV. Then we evaluate several contexts by assigning each a distinct starting position shift, increasing the shift in 100-token increments.~The average CVsim  drops sharply when RoPE encoding is used, whereas it is markedly reduced with CoPE as shown in Figure~\ref{fig:CoPE_robust1}.~However, CoPE cannot fully eliminate PIKVD of reuse contexts, as slight variations in prompt length across turns still introduce small but non-zero residual offsets. Although the residual drift in a single round is minimal, it may accumulate over multi-turn inferences.


\indent  To minimize the position-induced KV drift (PIKVD) in reusable contexts, we partition the LLM input into multiple chunks according to reuse-and-recompute criteria and assign each chunk a fixed positional-encoding range.~The positional encoding of context is learned through a dedicated algorithm and we devise a pre-training MLP like CoPE to analyze LLMs inputs, enabling the MLP to learn how to perform  positional encoding for both reuse and recompute chunks. Subsequently, we proceed to document the statistically prevalent positional encodings across chunks. When processing requests in similar scenarios, we directly apply these pre-recorded positional encodings to  chunks.We refer to this encoding scheme as \textbf{Chunked Contextual Position Encoding (CCPE)}.~As illustrated in Figure~\ref{fig:CCPEwithRoPE}, task-specific pre-training reveals that the positional pattern of the recomputed context remains invariant across inputs. We therefore designate it as chunk 1 and bind it to a fixed positional encoding, ensuring that variations in its length do not perturb the positional indices assigned to chunk 2. In contrast, under alternative schemes such as RoPE, any change in the length of chunk 1 inevitably shifts the positions allocated to chunk 2, undermining positional consistency.


\indent  As illustrated in Figure~\ref{fig:CCPEwithRoPE}, task-specific pre-training reveals that positional patterns of recomputed context remain invariant across inputs. We designate recomputed context as chunk 1 and bind it to a fixed positional encoding, ensuring that variations in its length do not affect positional indices assigned to chunk 2 (reusable context). In contrast, with RoPE, any change in chunk 1's length shifts positions allocated to chunk 2, undermining positional consistency.
The CCPE algorithm is presented in Algorithm~\ref{alg:ccpe}. During pretraining (lines 3-7), prompts of a single task type are encoded by CoPE, and a histogram identifies the most frequent encoding \(e^*\). Lines 8-14 partition the prompt into \(K\) ordered chunks labeled as \emph{reuse} or \emph{recompute}. During input processing (lines 15-23), new prompts are divided using the same scheme, with each chunk assigned its corresponding pretrained positional encoding, ensuring identical positional encodings across inference requests.
By assigning fixed positional ranges, CCPE reduces Position-Induced KV Drift (PIKVD) to near zero, addressing the positional encoding alignment challenge effectively.


% We explore whether the distinctive properties can be harnessed so that non-reusable contexts exert negligible influence on the positional encodings of reusable contexts.
% we use CVsim(section ~\ref{sec_WeightedCorrectionAttention})~as a metric to measures how similar a token’s KV remain after its positional encoding is shifted by a specified offset, relative to the token’s original KV. Then we evaluate several contexts by assigning each a distinct starting position shift, increasing the shift in 100-token increments.~The average CVsim  drops sharply when RoPE encoding is used, whereas it is markedly reduced with CoPE as shown in Figure~\ref{fig:CoPE_robust1} and we refer to the KV discrepancy that arises when the same context is assigned different positional encodings as \textbf{Position-Induced KV Drift (PIKVD)}.~However, CoPE cannot fully eliminate PIKVD of reuse contexts, as slight variations in prompt length across turns still introduce small but non-zero residual offsets. Although the residual drift in a single round is minimal, it may accumulate over multi-turn inferences.\\
%
%
\begin{figure}[t]
  \Description{This diagram shows how CCPE.}
 \includegraphics[height=0.25\textheight,width=0.9\linewidth]{sections/figures/section 4/CCPE.pdf}
  \caption{Overview of CCPE and comparation with RoPE.}
  \label{fig:CCPEwithRoPE}
\end{figure}
%
% \indent  To minimize the position-induced KV drift (PIKVD) in reusable contexts, we partition the LLM input into multiple chunks according to reuse-and-recompute criteria and assign each chunk a fixed positional-encoding range.~The positional encoding of context is learned through a dedicated algorithm and we devise a pre-training MLP like CoPE to analyze LLMs inputs, enabling the MLP to learn how to perform  positional encoding for both reuse and recompute chunks. Subsequently, we proceed to document the statistically prevalent positional encodings across chunks. When processing requests in similar scenarios, we directly apply these pre-recorded positional encodings to  chunks.We refer to this encoding scheme as \textbf{Chunked Contextual Position Encoding (CCPE)}.~As illustrated in Figure~\ref{fig:CCPEwithRoPE}, task-specific pre-training reveals that the positional pattern of the recomputed context remains invariant across inputs. We therefore designate it as chunk 1 and bind it to a fixed positional encoding, ensuring that variations in its length do not perturb the positional indices assigned to chunk 2. In contrast, under alternative schemes such as RoPE, any change in the length of chunk 1 inevitably shifts the positions allocated to chunk 2, undermining positional consistency.\\
% \indent  The CCPE algorithm is described in algorithm~\ref{alg:ccpe}, lines 3–7 demonstrate that a collection of prompts of a single task type is first encoded by CoPE and a histogram of encoding indices is constructed to identify the most frequent encoding \(e^*\). Lines 8–14 then partition the prompt’s context into \(K\) ordered chunks, alternatingly labeled as \emph{reuse} and \emph{recompute}. The dominant CoPE encoding \(e^*\) is partitioned according to the same chunking scheme and stored in the corresponding \(\textsf{Chunks}_{\mathrm{reuse}}\) and \(\textsf{Chunks}_{\mathrm{recompute}}\).
% Finally, Lines 15–23 illustrate the inputprocessing phase: new prompts are divided into chunks using the same scheme, and each chunk is assigned its corresponding pretrained positional encoding from the \(\textsf{Chunks}_{\mathrm{reuse}}\) and \(\textsf{Chunks}_{\mathrm{recompute}}\), thereby ensuring that reuse and recompute chunks  receive identical positional encodings across multiple inference requests.~Lines 21 and 23 allocate a larger positional budget to the recompute chunks and increment the positional indices of all subsequent chunks by one, thereby mitigating the PIKVD impact that length fluctuations in the recompute segment might impose on the reuse chunks and enhancing the overall robustness of the algorithm.~By assigning fixed positional ranges to both reusable and recomputed context chunks, CCPE reduces KV-cache PIKVD to near zero, whereas CoPE only mitigates the drift without eliminating it.
%
\begin{algorithm}[ht]
  \caption{Chunked Contextual Positional Encoding}\label{alg:ccpe}
  \begin{algorithmic}[1]
    % ==== Pretraining Phase ====
    \Statex \textbf{Pretraining Phase:} 
    \State   Require $\mathcal{P}$: set of prompts for one task; 
             $K$: total number of chunks; 
             $\mathcal{R}$: indices of chunks to reuse
    \State Initialize histogram $H \leftarrow 0^M$
    % , \quad max length tracker $L \leftarrow 0^K$
    \ForAll{$p \in \mathcal{P}$}
      \State $e \gets \textsf{CoPEEncode}(p)$ 
      \EndFor
    \State $e^* \gets \arg\max_e H[e]$ \Comment{Most frequent CoPE encoding}
    \State Store $(e^*)$ for later reuse
    % ==== Chunk Role Assignment ====
    \Statex \textbf{Chunk Role Assignment:}
    \For{$i = 1$ \textbf{to} $K$}
      \If{$i \in \mathcal{R}$}
        \State Mark chunk $c_i$ as \emph{reuse} \Comment{Determined by the prompt template.}
      \Else
        \State Mark chunk $c_i$ as \emph{recompute} \Comment{Determined by the prompt template.}
      \EndIf
    \EndFor

    % ==== Input Processing Phase ====
    \Statex \textbf{Input Processing Phase:}  
    \State Require new prompt $p_{\text{new}}$, $e^*$, $L$
    \State divide $p_{\text{new}}$ into $K$ chunks $\{c_1, \dots, c_K\}$
    \For{$i = 1$ \textbf{to} $K$}
      \If i in $\mathcal{R}$
        \State Assign positional encoding $e^*[i]$ to all tokens in chunk $c_i$
      \EndIf
      \State Assign positional encoding $e^*[i]$ $+$ 1 to all tokens in chunk $c_i$
    \State From $e^*[i+1]+1$ to $e^*[i+n]+1$.
    \EndFor
  \end{algorithmic}
\end{algorithm}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Weighted Correction  Attention}
\label{sec_WeightedCorrectionAttention}
%
With CCPE addressing positional encoding, our next focus is efficiently computing cross-attention between reused and recomputed contexts. To avoid full recomputation, we refresh only a strategically selected subset of cached KVs from reusable contexts.

Our key observation comes from analyzing KV cache behavior across model layers. As shown in Figure~\ref{fig:ckv}, cosine similarity between KVs of adjacent layers starts relatively low in shallow layers but increases steadily, reaching very high values in deeper layers. This indicates tokens' KVs have moderate similarity in adjacent shallow layers but become nearly identical in adjacent deep layers.
%
\begin{figure}[t]
  \includegraphics[width=0.95\linewidth]{sections/figures/section 4/CKV.pdf}
  \caption{Cross‑layers KV Cache Similarity.}
    \Description{Line plot showing that cosine similarity between cached
  and recomputed KV rises from ~0.2 in early layers to >0.9 in deep layers
  for all three datasets.}
  \label{fig:ckv}
\end{figure}
%
\begin{figure}[htbp]
  \centering
%----- 上方子图 -------------------------------------------------
  \begin{subfigure}{0.9\linewidth}
    \centering
    \includegraphics[width=\linewidth]{sections/figures/section 4/topk&CVsim.pdf} % ← 替换为实际图片
    \caption{Impact of Top-k Ratio and CVsim threshold on $\Delta$F1 Score.}
    \label{fig:subA}
  \end{subfigure}
  \begin{subfigure}{0.9\linewidth}
    \centering
    \includegraphics[width=\linewidth]{sections/figures/section 4/Weighted Correction Attention.pdf} % ← 替换为实际图片
    \caption{Workflow of Weighted Correction Attention.}
    \label{fig:subB}
  \end{subfigure}
  \caption{Overview of Weighted Correction Attention：(a) The impact of the top-k ratio and CVsim threshold on generation quality suggests setting top-k = 0.26 and CVsim = 0.12 as recommended values.(b) Architectural design of Weighted Correction Attention, illustrating both the intra-layer mechanism and the information flow across successive layers.}
  \label{fig:two-vertical}
\end{figure}
%
Based on this analysis, we propose Weighted Correction Attention, which operates in two main stages:
\begin{enumerate}
  \item \textbf{Select top-k tokens.}  
    In layer~1, we recompute the KVs for all reusable contexts. For each token \(i\), we compute the squared deviation \(d_i = \lVert V^{\mathrm{recompute}}_i - V^{\mathrm{reuse}}_i \rVert^2\), define the index set \(S = \{i \mid d_i > 0\}\), rank the scores \(\{d_i\}_{i \in S}\) in descending order and select the top-\(k\) tokens, denoting their index set by \(S_k \subseteq S\),~as shown in Figure~\ref{fig:subB} ~\ding{172} and ~\ding{173}.
  \item \textbf{Similarity-Gated Weighted Fusion.}  
   For each layer \(i>1\), we recompute only the tokens in \(S_k\), fuse the recomputed and cached KVs with deviation‐aware weights, and re‐evaluate their cosine similarity ckv. Every four layers, we set a similarity threshold \(\tau\); if for any token \(j\in S_k\) its \emph{CVsim} \(<\tau\), we remove \(j\) from \(S_k\) and \(S\),~then add to \(S_k\) the token \(m\in S\setminus S_k\) with the largest deviation score \(d_m\),~as shown in Figure~\ref{fig:subB} ~\ding{174} and ~\ding{175}.
\end{enumerate}


The workflow of Weighted Correction Attention is illustrated in Figure~\ref{fig:subB}. Algorithm~\ref{alg:wca-lite} provides additional implementation details. In the initialization phase (Lines 1-6), the algorithm compares each token's cached KV with its corresponding recomputed KV and collects the indices of all tokens with differing representations into candidate set $S$. It then selects the $k$ tokens with the largest discrepancies to form set $S_k$ and computes a fusion weight $\alpha_i$ for each selected token that quantifies the magnitude of discrepancy between its cached and recomputed KV.

During the similarity-gated weighted fusion phase (Lines 8-16), for each token $i \in S_k$, the algorithm recomputes the KV with respect to the unreusable contexts associated with it. The recomputed and cached KVs are then fused according to weight $\alpha_i$. After processing every four layers, the algorithm evaluates the cosine similarity between recomputed and reused KVs using the following metric as ~$\mathrm{CVsim}_i(reuse, recompute)$~This equation quantifies the extent to which the attention representation of token $i$ has been restored. If the similarity score for token $i$ falls below a predefined threshold $\tau$ (indicating sufficient convergence), the algorithm removes $i$ from $S_k$ and promotes to $S_k$ the token from $S \setminus S_k$ that exhibits the largest remaining discrepancy.

Both the CVsim threshold and the proportion of tokens selected by the top-k strategy significantly influence the generation quality of the LLM. We conducted a preliminary study comparing the change in F1 score obtained by tuning these two parameters against the baseline of fully recomputing the entire input. The results, shown in Figure~\ref{fig:subA}, suggest optimal values of 0.12 for the CVsim threshold and 0.26 for the top-k ratio (i.e., recomputing 26\% of the tokens).

% For additional details, please see section ~\ref{CVsim}.
\begin{algorithm}[!t]
\caption{Weighted Correction Attention}\label{alg:wca-lite}
\small
\begin{algorithmic}[1]
\Require cached KV $\{K_i^{\mathrm{reuse}},V_i^{\mathrm{reuse}}\}_{i=1}^N$, 
         total layers $L$, threshold $\tau$, stability $\varepsilon$, compute fusion weight $\alpha_i$
\State \textbf{(1) Initialization – Layer 1:}
\For{$i=1,\dots,N$}  \Comment{full recompute on entire prompt}
  \State $d_i \gets \lVert V_i^{\mathrm{recompute}} - V_i^{\mathrm{reuse}}\rVert_2$ and compute $\alpha_i$
\EndFor
\State $S   \gets \{\, i \mid d_i > 0 \,\}$      \Comment{indices with positive deviation}
\State $S_k \gets \text{Top-}k \text{ indices in } S \text{ ranked by } d_i$
\State \textbf{(2) Similarity-Gated Weighted Fusion - Layer $2$ to $L$:}
\For{$\ell = 2 \,\mathbf{to}\, L$}
  \ForAll{$i \in S_k$}
    \State V_i \gets \alpha_i\,V_i^{\mathrm{recompute}} \;+\; (1-\alpha_i)\,V_i^{\mathrm{reuse}}(same\ to \ K_i)$
    \State  $\(\alpha_i \gets \frac{\lVert V^{\mathrm{recompute}}_i - V^{\mathrm{reuse}}_i \rVert^2}{\lVert V^{\mathrm{reuse}}_i \rVert^2}\)$
    \If{ i \bmod 4 = 0} \Comment{every four layers, apply gating}
      \State $c_i \leftarrow
       \mathrm{CVSim}\!\bigl(
         V_i^{\mathrm{recompute}},\,
         V_i^{\mathrm{reuse}}
       \bigr)$ \Comment{}
      \If{$c_i < \tau$}
        \State remove $i$ from $S_k$
        \State $S_k \leftarrow \{\,m \in S \setminus S_k\,\}$
    \EndIf
  \EndFor
\EndFor
\end{algorithmic}
\end{algorithm}
% 
\begin{figure}[!htbp] % 星号(*)表示跨双栏
  \centering
  \includegraphics[width=0.49\textwidth,height=0.23\textheight]{sections/figures/section 4/PagedAttention_opt.pdf} % 调整width比例适应页面
  \caption{Compared with the base version of PagedAttention, CacheSlide extends the relocate and overwrite operations.} % 标题描述
  \label{fig:pagedattention_opt} % 引用标签
\end{figure}
%
% \indent 
% In brief,~Weighted Correction Attention  first selects a subset of tokens for recomputation rather than applying full attention, these tokens attend only to the unreusable portion of the context that pertains to them. The resulting KV is then combined with the cached KV through an appropriate weighting scheme to form recomputed KV. Leveraging the increasing similarity of KV across adjacent layers, Weighted Correction Attention subsequently refines the set of tokens chosen for recomputation.More importantly, \textbf{the attention over these reusable contexts must be restricted to their mutual interactions}. otherwise, it is impossible to determine whether the discrepancy between the recomputed and reused KVs arise from the unreusable context.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Relocation and Overwrite in PagedAttention}\label{PagedAttention_opt}
LLMs operate layer by layer: each layer first loads the KV cache and then writes selected tokens’ KVs during its prefill phase. Base pagedAttention allocates KV pages only once per layer sized to the prompt length,~ so the pages are already fully occupied by KV cache and the recomputed KVs. ~As a result, writing the selected tokens’ KVs into KV cache of layer i must \textbf{wait} until the KV cache has been loaded. Furthermore, additional context is occasionally appended to the prompt suffix (see Section \ref{back_1}),which will later become reusable. The Weighted Correction Attention  must compute these KVs with the original KV cache. Consequently, writing the selected tokens’ KVs into KV cache cannot begin until the appended context’s KVs are available. This workflow-- \emph{loading} the KV cache, \emph{computing} the appended KVs and then \emph{writing} the selected tokens’ KVs under the base pagedAttention inevitably increases the TTFT.\\
\indent To reduce TTFT,~we preallocate extra memory pages from layer 2 to n based on the number of tokens selected in layer 1
and relocate the selected tokens’ KVs from original pages to extra memory pages. As shown in Figure ~\ref{fig:pagedattention_opt}~\ding{172}, by relocating the selected tokens’ KVs, we break the two blocking dependencies: the layer i can the load KV cache and get the selected tokens’ KVs in pipeline and get the selected tokens’ KVs  can pipeline with computating of the appended context’ KVs. Consequently, loading the KV cache and computing the appended KVs by KV cache can now proceed in parallel with writing the selected tokens’ KVs. ~However, relocating the selected tokens’ KVs lead their original KV cache slots unused. To curb this waste, we repurpose the vacated space during decoding, writing the newly generated tokens’ KVs  into them as shown in Figure~\ref{fig:pagedattention_opt}~\ding{173}.

\noindent \textbf{Implementation}:~Our implementation is based on vLLM 0.8.5~\cite{vllm0.8.5}.~In \emph{PagedAttention.\_init\_cache}, extra memory pages are preallocated for layers 2 to n based on the number of tokens selected in the first layer (via \emph{KVCacheManager.append\_slot}) and these pages are set aside for the selected tokens’ KVs. Then, in \emph{WeightedCorrectionAttention}, \emph{KVCacheManager.promote} is invoked to copy the selected tokens’ KV data from the original pages into the newly allocated pages with the \emph{slot\_mapping} updated accordingly. This relocation allows writing the selected tokens’ KVs to proceed in parallel with KV cache loading and appended context computation, thereby removing the former sequential dependencies. Once the selected tokens’ KVs have been moved, the freed slots in the original pages can be reused for newly generated tokens by calling \emph{KVCacheManager.append\_slot(overwrite=True)} or \emph{write\_to\_kv\_cache} with the \emph{overwrite} mechanism, reducing allocation overhead and lowering TTFT through continued reuse of these freed slots during decoding.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Controller and Cache Engine of CacheSlide}
% % 
% The proposed system as shown in Figure~\ref{fig:system_overview} integrates task dispatching controller, cache engine responsible for system scheduling and KV-cache management described as follows:\\
% \textbf{task dispatching controller:} 
% The Task Dispatching Controller receives a user prompt, it divides the prompt into chunks based on reuse and recompute. ~As shown in Figure~\ref{fig:system_overview} ~\ding{172} the controller then send reuse chunks to the Cache Management Component and sends the recompute chunks to LLMs as shown in  Figure~\ref{fig:system_overview}~\ding{175}. ~After the LLM completes the current inference, it sends appending KV to KV Cache Store module as shown in Figure~\ref{fig:system_overview}~\ding{176} and  ~\ding{172}.\\
% \textbf{cache engine:} 
% ~The cache engine is a retrieving reusable KV and storing newly generated KV module via computing prompt hash to ensure consistent identification and reuse of the same prompt context. ~Upon receiving a KV retrieval request from the Task Dispatching Controller, the cache engine hashes the input prompt to locate and fetch any reusable KVs from the storage hierarchy. The underlying storage adopts a conventional hot and cold tiering policy: hot data reside in DRAM, whereas cold data are stored on SSD; This design is already widely used, and we therefore do not detail it further in our work. These retrieved KV are subsequently transmitted to the LLMs for context initialization during the prefill phase as Figure~\ref{fig:system_overview}~\ding{172}, ~\ding{173} and ~\ding{174}. Conversely, when processing an append KV request, the system stores the KV by hash key. The process is schematically illustrated as Figure~\ref{fig:system_overview}~\ding{177}, ~\ding{172} and ~\ding{173}.\\ 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%













==> sections/motiv.tex <==
\section{Preliminaries and Motivation}\label{sec3}
%
This section introduces our defined RPDC(relative-position-dependent caching), presents preliminary experiments that analyze limitations of existing KVCache reuse strategies in agent applications, illustrates the position-induced KV drift phenomenon, preliminary of Window Padding, and identifies the key challenges that motivate our approach.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Relative-Position-Dependent Caching}\label{PRDC}
Recent systems have mitigated prefill overhead by identifying identical context across different LLM inputs, caching key-value (KV) pairs, and reusing them across subsequent requests. Context reuse demonstrates significant benefits in multi-turn inference tasks as discussed in Section~\ref{back_2}. Figure~\ref{fig:Reuse_Proportion_of_rpdc} illustrates that the proportion of reusable context length relative to total prompt length is high. ~Therefore, reusing the KVCache represents the optimal approach for performance optimization.~More importantly, as shown in Figure~\ref{fig:back_2}~\ding{172}, we \textbf{cannot simply swap the fixed and updated segments and reuse the KVCache via prefix caching}, Since the prompt head generally attracts more attention~\cite{attention_head,attention_head_1}, representative designs (e.g., MemGPT) position recent memories(Working Window) close to the head instead of FIFO historical content to maintain inference quality.~Similarly, in SWE-agent a widely used code-debugging agent with multiple updated slots~\ding{173} the updated slots cannot be swapped with immutable segments~\ding{174}, as such reordering changes program semantics and breaks data dependencies  (e.g., if Updated Slot 1 produces a run-time parameter later consumed by Immutable 1, moving the slot to the suffix prevents Immutable 1 from receiving it).\\
\indent We  We define Relative-Position-Dependent Caching (RPDC) as a class of scenarios involving KVCache reuse, such as those in agent prompts, where context is composed of multiple segments whose relative order remains fixed(\emph{arbitrary reordering incurs substantial degradation}), while segments between these reusable context segments are continuously updated.~
%
%
\subsection{Limitation of PDC \& PIC Implementations for RPDC}\label{sec:LimitofPIC_PDC} //本身的问题写出来
Current mainstream Position-Dependent Caching (PDC) implementations, ContextCache and PromptCache (Section~\ref{sec_2.3}), are ineffective for RPDC scenarios. PromptCache assigns buffers to reusable segments, but in RPDC, variable-length non-reused segments cause buffer expansion and excessive storage consumption.~Furthermore, PromptCache precomputes KVs without knowledge of other reusable contexts, ignoring critical cross-attention between reused segments, resulting in low precision and storage inefficiency.~For instance, ContextCache only reuses KVCaches when inputs share identical prefix prompts. 
% As Figure~\ref{benefit_reuse_suffix} illustrates, only system prompts serve as common prefixes, constituting less than 20\% of entire prompts. 
~This limitation yields minimal computational savings and negligible TTFT reduction in RPDC scenarios.

Position-Independent Caching (PIC) implementations, such as CacheBlend and EPIC, similarly underperform for RPDC. ~Since reused contexts' starting positional indices reset to zero, \emph{significant misalignment occurs between cached KVs and their intended positions in original inputs}. ~This misalignment creates incorrect KVCaches that cannot be arithmetically adjusted. ~Even when extracting tokens for recomputation, accurate attention calculation remains impossible: token $i$ must attend to positions $0$ through $i-1$, but some KVs come from reused contexts with incorrect positional information. These methods also redundantly recompute cross-attention for reusable segments, further reducing efficiency.~They preselecte some tokens to recompute
(\S~\ref{sec_2.3}) to recover attention.~However, in multi-head attention of transformer, \emph{different heads attend to different tokens, and the model’s output is fusing  the per-head results}~\cite{mutil-head_2,mutil-head}.~During decoding, the set of heads that contribute most to the output varies with the context at each step~\cite{mutil-head_3,mutil-head_4}.~Since which tokens most affect the output becomes clear only at the decoding stage, prefill-phase token-subset preselection cannot ensure stable accuracy. 
%
\subsection{Position-Induced KV Drift and
 Window Padding}\label{sec:PIKVD_and window_padded}
%
\begin{figure}[t]
  \includegraphics[width=0.98\linewidth]{sections/figures/section 3/PIKVD.pdf}
  \caption{Compared with RoPE, CoPE achieves better alignment between cached and real positions during KVCache reuse, yielding a shallower mapping slope and thereby substantially reducing the positional discrepancy  ($\Delta \mathrm{pos}$ ).}
   \vspace{-3ex}
  \label{fig:PIKVD_and_padding}
\end{figure}
%
% 
\begin{figure}[t]
\includegraphics[width=0.98\linewidth,height=3cm]{sections/figures/section 3/PIKVD&Padding.pdf}
  \caption{(a) shows that as the positional shift increases (0–1000 tokens), CKSim with RoPE drops by $>90\%$, whereas CKSim with CoPE decreases by only 28\%. (b) shows that applying window padding(1K/2K/3K) yields $>78.1\%$ lower F1 score relative to baseline inference at the same reasoning rounds.}
   \vspace{-3ex}
  \label{fig:expofCKsim}
\end{figure}
%
% 
Current KVCache reuse methods(PIC) produce positional indices misalignment compared to recomputation.  To quantify the impact of positional shifts on KV similarity between recomputed and reused KVCaches, we implement the well-known CKsim~\cite{CKV_1,CKV_2}.
\[
\mathrm{CKsim}(reuse,recompute)=\frac{1}{H}\sum_{i=1}^{H}\frac{K_i^{(\mathrm{recompute})}\cdot K_i^{(\mathrm{reuse})}}{\lVert K_i^{(\mathrm{recompute})}\rVert\lVert K_i^{(\mathrm{reuse})}\rVert}
\]

We evaluate CKSim by MemGPT~\cite{MemGPT} on ShareGPT~\cite{ShareGPT} dataset by constructing, for a each user, a static historic memory(MemHistory). ~We proceed as follows:
\begin{enumerate}
  \item Using RoPE, encode MemHistory and obtain the baseline KVCache as \emph{KVCache 0}.
  \item For prefix window(i.e., the length of the context preceding MemHistory) sizes \(i \in \{100,200,300,\ldots\}\) (step size: 100 tokens),  prepend a prefix of length \(i\) to MemHistory and run a partial prefill(Only the positional information of MemHistory is prefilling; attention on the prefix is not computed) to obtain \emph{KVCache i}.
  \item Compute \(\mathrm{CKSim}\) between  \emph{KVCache i} and \emph{KVCache 0}.
  \item Replace RoPE with CoPE and repeat steps~(1)--(3).
\end{enumerate}

\indent As shown in Figure~\ref{fig:expofCKsim}~(a), we observe that RoPE exhibits a more pronounced decline in CKSim, whereas CoPE maintains comparatively stable CKSim. ~We define \textbf{Position-Induced KV Drift (PIKVD)} as the discrepancy in KVCache similarity  for the same text that is attributable to differences in positional encodings.~As shown in Figure~\ref{fig:PIKVD_and_padding}~\ding{172},when the length of the update segment changes, the real positional indices of the fixed segment can diverge substantially from those stored in the KVCache, because RoPE assigns a position index to every token(For example, after the update, the true starting positions in the KVCache are 251 and 451, whereas the cached positions remain at 101 and 401). ~Under the same update length, CoPE markedly reduces the positional offset of the fixed segment. For example, in Figure~\ref{fig:PIKVD_and_padding}~\ding{173}, the offset $\Delta\mathrm{pos}$ decreases, with the fixed segment’s starting positions shifting from (10, 21) to (9, 20). ~At a deeper reason, as shown in Figure ~\ref{fig:PIKVD_and_padding}~\ding{174}, when the starting positions of one context shift, RoPE exhibits a steeper change in positional indices because it maps each token to a unique position, whereas CoPE varies more smoothly since multiple tokens can share a single position.\\
\noindent \textbf{Window Padding in RPDC:}~In order to minimize the PIKVD gap between reused and recomputed KVCaches, we enforce a fixed-size update window for the updated segments (capping its max token count),~so that the positions of the fixed segments  remain invariant, as shown in Figure~\ref{fig:PIKVD_and_padding}~\ding{172} window padding. ~Using MemGPT, we fix the  working window to 1K,2K and 3K tokens, after multiple reasoning rounds (as shown in Figure~\ref{fig:expofCKsim}~(b)), window-padded inference attains markedly lower accuracy than the baseline inference(not set window-padded), indicating that enforcing a fixed-length update segment can cause the loss of critical information across inferences(working window=1K) or larger window(working window=3K) padding increases the PIKVD of the fixed segment’s KVCache.~In window-padded experiments, we observe that fixing the updated-segment length enables lossless reuse of KVCaches for interactions involving fixed segments, because their positional indices are invariant and the content of the attended fixed segments does not change and it motivates reusing cross-attention to fixed segments.
%

%
\subsection{Challenges of RPDC}\label{ChallengesofPRDC}
Building on the above, in the RPDC setting our primary design objective is to maximize \textbf{caching  attention} for the reused segments \textbf{without constraining the update-segment length} by increasing the \textbf{positional similarity} of the fixed segments between the cached and recomputed passes.~This poses four key challenges:\\
%
\noindent \textbf{C1: Positional Encoding Alignment.} Maintaining the positions of stored KVCaches  as close as possible to the positions of the same contexts would occupy if recomputed in the LLM’s input facilitates efficient lossless reuse in KVCaches (\S~\ref{sec:PIKVD_and window_padded}).~However, updated segments occur at different positions across inputs, causing the cached encoding scheme to disassign recomputed schema.~The critical objective is to maintain positional alignment as closely as possible, instead of using window padding, which can markedly reduce generation quality.

\noindent \textbf{C2: Efficient Attention Recovery.}?? When reusing the KVCache, current methods(\S~\ref{sec:LimitofPIC_PDC} ) must perform full attention recomputation to recover proper attention mechanisms. ~This necessitates additional computation to reestablish attention relationships among reusable contexts, even when these contexts attend solely to other reusable contexts rather than to non-reusable contexts. ~Therefore, the goal is to recover attention mechanisms for KVCaches while minimizing redundant computation among reusable contexts.\\
%
\begin{figure*}[t] % 星号(*)表示跨双栏
  \centering
  \includegraphics[width=0.95\textwidth]{sections/figures/section 4/OverView.pdf} % 调整width比例适应页面
  \caption{Block diagram of proposed CacheSlide system workflow} % 标题描述
  \label{fig:system_overview} % 引用标签
\end{figure*}
%
\noindent \textbf{C3: Limitations of PagedAttention.} ??
To restore inter-segment self-attention between fixed and updated segments, we must (i) write back the recomputed KVs for the fixed segments (update-write) and (ii) load existing KVCaches layer by layer. ~However, PagedAttention performs one-shot, per-layer allocation of a fixed number of pages for the current input without reserving spare pages, which precludes directly merging recomputed KVs. Consequently, write-back must be preceded by loading the existing caches, creating a serialized load-then-write path that increases TTFT (time to first token). Compared with baseline page management that requires only a single write, RPDC’s attention recovery triggers both loading and write-back, thereby incurring additional latency. ~Under GPU/host memory pressure, the KVCache inevitably spills to SSDs. ~During attention restoration, ~new KVs must be written to KVCache; however, existing methods \textbf{lack dirty-page awareness} and cannot determine whether a KV-cache page will be modified. ~Consequently, when such pages spill to SSDs, trigger random write patterns on SSDs and raising prefill latency.\\
\textbf{Summary.} ~Without altering the RPDC prompting paradigm, designing a new KVCache reuse scheme that achieves high accuracy, low latency, low compute cost, and storage efficiency has become a pressing design challenge. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
3.1 PDC
3.2 limit of pic 
3.3 WP 
3.4 RPDC

